Windows into Geometric Events: Data Structures for Time-Windowed Querying of Temporal Point Sets

We study geometric data structures for sets of point-based temporal events, answering time-windowed queries, i.e., given a contiguous time interval we answer common geometric queries about the point events with time stamps in this interval. The geometric queries we consider include queries based on the skyline, convex hull, and proximity relations of the point set. We provide space efficient data structures which answer queries in polylogarithmic time.

==> previous.tex <==
\subsection{Previous Related Work}

First, we note that windowed querying is different than dynamic computational
geometry.
Dynamic computational geometry is a rich research area,
where we wish to maintain a data structure over a set of geometric objects,
subject to insertions, deletions, and queries.
(E.g., see~\cite{ct-dacg-92,de2008computational}.)
In windowed geometric querying, the objects are static events and we are
interested in querying geometric attributes about the set over a window of
time.

Also note that this is not the same as batched dynamic querying, where the
queries are known in advance 
(e.g., see~\cite{Edelsbrunner1985515}).
In window-based querying, we don't know the time windows or the queries being
requested in those windows in advance.

Similarly, windowed querying is also not the same as off-line geometric
querying (e.g., see~\cite{Agarwal199165,hs-olmpc-96}), where a sequence of
insertions and deletions is given in advance and then queries are performed
``in the past'' with respect to this sequence.
Likewise, windowed querying is not the same as 
the persistent data structure framework
(e.g., see~\cite{Driscoll198986}), where a sequence of insertions and
deletions is performed on a data structure in an online fashion, with that
data structure optimized to allow for queries coming later that are done
``in the past.''
Windowed data structures allow for different ``starting times'' for such
sequences of operations, whereas these previous approaches always have to
start at time~$0$.

Perhaps the closest previous work with respect
to geometric querying is that on concatenable structures for 
ordered decomposable problems
(e.g., see~\cite{Grossi19991,Vankreveld1994130}).
In this framework, a set of objects is given in some order,
such as $x$-coordinates or a time coordinate,
and geometric 
queries are performed on this set, subject to splits and merges along one
of these dimensions.
Such a structure can be used to solved a 
windowed geometric query, then, for a time window $[t_1,t_2]$, by 
splitting the structure at $t_1$ and at $t_2$, and then asking queries on the
resulting structure.
Previous work on this approach has been primarily focused on bucketing
techniques, however, which do not result in the same fast running times that
we are able to achieve.
[xxx PLEASE DOUBLE-CHECK ME xxx]

The SODA paper \cite{BanDubEppSmy-SODA-13}

